VLPose: Bridging the Domain Gap in Pose Estimation with Language-Vision Tuning

Thanks to advances in deep learning techniques, Human Pose Estimation (HPE) has achieved significant progress in natural scenarios. However, these models perform poorly in artificial scenarios such as painting and sculpture due to the domain gap, constraining the development of virtual reality and augmented reality. With the growth of model size, retraining the whole model on both natural and artificial data is computationally expensive and inefficient. Our research aims to bridge the domain gap between natural and artificial scenarios with efficient tuning strategies. Leveraging the potential of language models, we enhance the adaptability of traditional pose estimation models across diverse scenarios with a novel framework called VLPose. VLPose leverages the synergy between language and vision to extend the generalization and robustness of pose estimation models beyond the traditional domains. Our approach has demonstrated improvements of 2.26% and 3.74% on HumanArt and MSCOCO, respectively, compared to state-of-the-art tuning strategies.

==> tables/decoder.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Vision-Language Decoder}. We conduct ablation experiments on pose decoder structures, which encompasses the baseline decoder (None), injector decoder (in), extractor-injector decoder (ex-in), and dual extractor-injector decoder (2-ex-in). Bold and underlined text signify the best and second-best results. Gray background indicates our selection.}
\setlength{\tabcolsep}{3mm}
\small
\begin{tabular}{c|ccccc}
\toprule
Model & AP & AP50 & AP75 & AR & AR50 \\
\midrule
None & 36.45 & 52.60 & 38.56 & 43.12 & 59.28 \\
in & 36.93 & 52.86 & 39.34 & 43.48 & \uline{59.55} \\
ex-in & \uline{37.13} & \uline{53.08} & \textbf{39.47} & \uline{43.63} & 59.48 \\
\rowcolor{gray!20} 2-ex-in & \textbf{37.16} & \textbf{53.14} & \uline{39.43} & \textbf{43.76} & \textbf{59.90} \\
\bottomrule
\end{tabular}
\label{tab:decoder}
\end{table}

==> tables/encoder.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Text encoder}. Ablation experiments on text encoders including albef and blip.}
\setlength{\tabcolsep}{2.8mm}
\small
\begin{tabular}{c|ccccc}
\toprule
Model & AP & AP50 & AP75 & AR & AR50 \\
\midrule
None & 36.45 & 52.60 & 38.56 & 43.12 & 59.28 \\
albef \cite{albef}& 36.78 & 52.63 & 38.78 & 43.49 & 59.40 \\
\rowcolor{gray!20}blip \cite{blip}& \textbf{37.16} & \textbf{53.14} & \textbf{39.43} & \textbf{43.76} & \textbf{59.90} \\
\bottomrule
\end{tabular}
\label{tab:encoder}
\end{table}


==> tables/matcher.tex <==
\begin{table}[t]
\centering
\caption{Ablation experiments of multi-head attention input configurations in the relation matcher, including text feature $T$, image feature $E$, the concatenation of both features $[E, T]$, and the concatenation of image feature and cosine similarity of the features $[E, E\cdot T]$.}
\setlength{\tabcolsep}{2.7mm}
\small
\begin{tabular}{c|ccccc}
\toprule
$K=V$ & AP & AP50 & AP75 & AR & AR50 \\
\midrule
None & 36.45 & 52.60 & 38.56 & 43.12 & 59.28 \\
$T$ & 36.58 & 52.98 & 38.68 & 43.23 & 59.70 \\
$[E, E\cdot T]$ & 36.74 & 53.02 & 38.74 & 43.49 & \textbf{59.91} \\
\rowcolor{gray!20}$[E, T]$ & \textbf{37.16} & \textbf{53.14} & \textbf{39.43} & \textbf{43.76} & 59.90 \\
\bottomrule
\end{tabular}
\label{tab:matcher}
\end{table}

==> tables/param.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.5mm}
\small
\begin{tabular}{c|c|cccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{finetune} & \multicolumn{4}{c}{Size} \\
 &  & Small & Base & Large & Huge \\
 \midrule
\multirow{2}{*}{ViTPose \cite{vitpose}} & visual prompt & 2.65 & 4.22 & 5.26 & 6.30 \\
 & last layer & 4.40 & 11.29 & 17.85 & 25.98 \\
   \midrule
\rowcolor{gray!20}VLPose & visual prompt & 3.74 & 6.75 & 10.48 & 14.05 \\
\bottomrule
\end{tabular}
\caption{Parameters, measured in megabytes (MB), of different finetuning methods including visual prompt tuning and last-layer tuning.} % \textbf{Parameters}. 
\label{tab:param}
\end{table}

==> tables/prompt.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Text prompt}. Ablation experiments of text prompts, including random prompts, fixed prompts, and style prompts.}
\setlength{\tabcolsep}{2.5mm}
\small
\begin{tabular}{c|ccccc}
\toprule
Prompt & AP & AP50 & AP75 & AR & AR50 \\
\midrule
None & 36.45 & 52.60 & 38.56 & 43.12 & 59.28 \\
Random & 36.74 & 52.77 & 38.90 & 43.30 & 59.36 \\
Fixed prompt & 36.76 & 52.78 & 39.20 & 43.45 & 59.52 \\
\rowcolor{gray!20}Style prompt & \textbf{37.16} & \textbf{53.14} & \textbf{39.43} & \textbf{43.76} & \textbf{59.90} \\
\bottomrule
\end{tabular}
\label{tab:prompt}
\end{table}

==> tables/wo_matcher.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Relation Matcher}. Ablation experiments of relation matcher. `w/o text' is the naive baseline without integrating text tokens. `w/o matcher' simply concatenates text and image tokens. Bold text signifies the best results. Gray background indicates our selection.}
\setlength{\tabcolsep}{2.3mm}
\small
\begin{tabular}{c|ccccc}
\toprule
$K=V$ & AP & AP50 & AP75 & AR & AR50 \\
\midrule
w/o text & 36.45 & 52.60 & 38.56 & 43.12 & 59.28 \\
w/o matcher & 36.54 & 52.98 & 38.48 & 43.09 & 59.34 \\
\rowcolor{gray!20}w matcher & \textbf{37.16} & \textbf{53.14} & \textbf{39.43} & \textbf{43.76} & \textbf{59.90} \\
\bottomrule
\end{tabular}
\label{tab:wo_matcher}
\end{table}

==> versions/decoder.tex <==
\subsection{Vision-Language Decoder}
\label{sec:decoder}
By feeding the image feature and text feature into the relation matcher, we obtain the image-text relationship matrix \(R \in \mathbb{R}^{P \times C}\), which is then input into the pose decoder. In this section, we will outline the structure of the pose decoder, encompassing both the traditional pose estimator and our proposed vision-language decoder. The architectural details are depicted in \cref{fig:decoder}.

\paragraph{Baseline.} The baseline Decoder is comprised of two deconvolution blocks, each containing a deconvolutional layer, followed by batch normalization \cite{bn}, and activation using the Rectified Linear Unit (ReLU) \cite{relu}.   Following established conventions from prior studies \cite{zhang2020empowering, baseline}, each block executes an upsampling operation, effectively doubling the size of the feature maps. Subsequently, a convolution layer with a $1\times1$ kernel size is employed to generate the localization heatmaps for the keypoints. The specifics of the architecture are visually represented in \cref{fig:decoder_baseline}. Mathematically, this process can be expressed as 
\begin{equation}\label{equ:decoder_baseline}
K_{b} = p(f_m(f_m(E))), 
\end{equation}
where $K_{b} \in \mathbb{R}^{\frac{H}{4} \times\frac{W}{4} \times N_k}$ represents the estimated heatmaps, with one heatmap produced for each keypoint, and $N_k$ denoting the total number of keypoints to be estimated. $E$ denotes the image feature. $p$ refers to the predictor, which consists of a $1\times1$ convolution layer. $f_m$ represents a decoder block, with the subscript $m$ serves to distinguish it as the main branch, setting it apart from the auxiliary branch, which will be discussed later.

\paragraph{Injector Decoder.} An injector decoder involves a simple method to inject image-text relationship knowledge into the traditional decoder. It combines the image feature $E$ with the image-text relation $R$ and subsequently feeds the combined information into the structure identical to the baseline, which comprises two decoder blocks and one predictor. \cref{fig:decoder_in} illustrates the design. The procedure can be formally represented as
\begin{equation}\label{equ:decoder_in}
K_{i} = p(f_m(f_m(E+R))), 
\end{equation}
where $p$ and $f_m$ denote the predictor and the decoder block.

\paragraph{Extractor-Injector Decoder.} Drawing inspiration from the successful developments within the field of dense prediction tasks \cite{vitadapter}, we have devised an approach tailored specifically for our vision-language decoder. The decoder is primarily composed of two branches, each consisting of 2 decoder blocks. The main branch is labeled as $f_m$, while the auxiliary branch is denoted as $f_a$. The image feature $E$ is first integrated with the image-text relation $R$ within the auxiliary branch. Subsequently, the resulting output from the auxiliary branch is collaboratively fed into the pose predictor along with the output from the main branch for pose predictor. The role of the auxiliary branch is to extract image features and inject relationship knowledge into the main branch, aiding in pose estimation through an extractor-injector mechanism. A visual representation of the architecture is in \cref{fig:decoder_ex_in}. The output of the main branch is as follows:
\begin{equation}\label{equ:decoder_ex_in}
K_{ei} = p(f_m(f_m(E)) + f_a(f_a(E+R))), 
\end{equation}

Since the main branch shares the same structure as the traditional pose decoder, it's evident that when $R$ equals 0 and the auxiliary branch weights are all zeros ($f_a$ weights), the VLPose estimator reverts to the baseline Pose decoder as \cref{equ:decoder_baseline}. Therefore, when we freeze the main branch and fine-tune the auxiliary branch, we can still preserve the capability of the original structure.

\paragraph{Dual Extractor-Injector Decoder.} Furthermore, we have advanced our approach by introducing a decoder that incorporates dual extractor-injector structure, which is graphically presented in \cref{fig:decoder_2_ex_in}. In this configuration, the image feature $E$ and the image-text relation $R$ are combined and fed into the main branch, while the auxiliary branch extracts the output of the first decoder block as:
\begin{equation}
    K'_{2ei} = f_m(E+R),
\end{equation}
where $K'_{2ei}$ is the inter output of the 1st main decoder block. Subsequently, the output from the auxiliary branch is combined with that from the main branch and jointly fed into the predictor as:
\begin{equation}\label{equ:decoder_2_ex_in}
    K_{2ei} = p(f_m(K') + f_a(K'+f_a(R))), 
\end{equation}
where $p$ denotes the predictor. $f_m$ and $f_a$ represent the main and auxiliary branch. 

The dual extractor-injector decoder combines the advantages of the extractor-injector decoder, offering the flexibility to restore pre-trained weights by simply setting $R$ to zero and omitting the auxiliary branch. This approach preserves the performance of pre-training while allowing for model fine-tuning. Moreover, the dual extractor-injector decoder introduces an elevated level of synergy and cooperation between the main branch and the auxiliary branch. This heightened interaction serves to augment the model's overall capacity, leading to more effective and robust performance across various tasks and domains. In \cref{sec:ab_decoder}, we execute a series of ablation experiments with the primary aim of empirically validating the advantages conferred by our extractor-injector structures when contrasted with conventional architectures. In the appendix, we further delve into additional strategies for fusing multi-modal knowledge. 

